Refined convergence for the Boolean model

In a previous work, two of the authors proposed a new proof of a well known convergence result for the scaled elementary connected vacant component in the high intensity Boolean model towards the Crofton cell of the Poisson hyperplane process. In this paper, we consider the particular case of the two-dimensional Boolean model where the grains are discs with random radii. We investigate the second-order term in this convergence when the Boolean model and the Poisson line process are coupled on the same probability space. A precise coupling between the Boolean model and the Poisson line process is first established, a result of directional convergence in distribution for the difference of the two sets involved is derived as well.

==> aptpub.cls.tex <==
\def\filename{aptpub.cls}
\def\fileversion{10}
\def\filedate{8 January 2004}
%% This is aptpub.cls, public version
%% Copyright (C) 2001 Applied Probability Trust.
%% Written by Stephen Webb.
%% Updated by Maria Kelly and by David Cruickshank
%% All rights reserved.
%% Copying of this file is authorized only if
%% you make absolutely no changes to your copy.
%%
\typeout{\filename\space v\fileversion, (C) Copyright Applied Probability Trust, \filedate}
\NeedsTeXFormat{LaTeX2e}
\ProvidesClass{aptpub}[2001/03/09]
\DeclareOption*{\PassOptionsToClass{\CurrentOption}{article}}
\ProcessOptions
\LoadClass[twoside]{article}
\RequirePackage{ifthen,calc}
\RequirePackage{amsbsy,amsfonts,amssymb,amsmath}
\RequirePackage{theorem}
%%
% The following sorts out the dimensions of the page
%%
\normalsize
\evensidemargin=0pt
\oddsidemargin=0pt
\hoffset=6pt
\voffset=30pt
\textwidth 375pt
\setlength{\textheight}{569.6788pt}
\headheight 11pt
\headsep 19pt
\footskip 24pt
\parindent 12pt
\topskip 10pt
\abovedisplayskip=10pt plus 2pt minus 8pt
\belowdisplayskip=10pt plus 2pt minus 8pt
\belowdisplayshortskip=5pt plus 3pt minus4pt
%
\renewcommand{\baselinestretch}{1.5}
%
%%
% The following are for list structures
%%
\renewenvironment{itemize}
                 {\begin{list}{$\bullet$}
                  {\setlength{\topsep}{6pt plus 2pt minus2pt}
                  \setlength{\partopsep}{0pt}
                  \setlength{\itemsep}{3pt}
                  \setlength{\parsep}{0pt}}
                 }{\end{list}}
%
\setlength{\topsep}{6pt plus 2pt minus2pt}
\setlength{\partopsep}{0pt}
\setlength{\itemsep}{3pt}
\setlength{\parsep}{0pt}
%%
% The page styles . . .
%%
% . . . for the first page
%%
\def\ps@firstpg{\let\@mkboth\@gobbletwo
\def\@evenhead{\hfil\crnotice{}}
\def\@oddhead{\hfil\crnotice{}}
\def\@evenfoot{{\small\textrm\hfil\thepage\hfil}}
\def\@oddfoot{{\small\textrm\hfil\thepage\hfil}}}
%%
% . . . and for subsequent pages
%%
\def\ps@myheadings{\let\@mkboth\@gobbletwo
\def\@evenhead{{\small\textrm\thepage}\hfill{\small\textrm{\uppercase{\authornamesa}}}}
\def\@oddhead{{\small\textit{\shorttitlea}}\hfill{\small\textrm\thepage}}
\def\@evenfoot{\rm\hfill}
\def\@oddfoot{\rm\hfill}}
%%
\pagestyle{myheadings}
%%
\newcommand{\shorttitlea}{Short title}
\newcommand{\shorttitle}[1]{\renewcommand{\shorttitlea}{#1}}
\newcommand{\authornamesa}{AUTHOR NAMES}
\newcommand{\authornames}[1]{\renewcommand{\authornamesa}{#1}}
%%
% Elements belonging to the title page
%%
\renewcommand\thefootnote{}
\renewcommand\footnoterule{\flushleft\raisebox{2pt}{\rule{42.68pt}{0.4pt}}}
\skip\footins=17.07pt
%
\newcommand{\crnotice}{\hfill{{\small\emph{Applied\ Probability\ Trust}\ (\today)}}}
%
\renewcommand{\today}
             {\number\day \space \ifcase\month\or
              January\or February\or March\or April\or May\or June\or
              July\or August\or September\or October\or November\or December
              \fi \space \number\year
             }
%%
% The title
%%
\renewcommand{\title}[1]
             {\thispagestyle{firstpg}
              \vspace*{9pt}
              \noindent\fontsize{11}{13}\selectfont\textbf{\uppercase{#1}}}
%%
% The author/institution:
%%
\newcommand{\authorone}[2][]{\hspace*{9pt}{\small\textrm{\uppercase{#2}},$^{*}$ \textit{#1}}\par}
\newcommand{\authortwo}[2][]{\hspace*{9pt}{\small\textrm{\uppercase{#2}},$^{**}$ \textit{#1}}\par}
\newcommand{\authorthree}[2][]{\hspace*{9pt}{\small\textrm{\uppercase{#2}},$^{***}$ \textit{#1}}\par}
\newcommand{\authorfour}[2][]{\hspace*{9pt}{\small\textrm{\uppercase{#2}},$^{****}$ \textit{#1}}\par}
\newcommand{\authorfive}[2][]{\hspace*{9pt}{\small\textrm{\uppercase{#2}},$^{*****}$ \textit{#1}}\par}
\newcommand{\authoronesame}[1]{\hspace*{9pt}{\small\textrm{\uppercase{#1}}\,$^{*}$ \textsc{and}}\par}
\newcommand{\authornostar}[2][]{\hspace*{9pt}{\small\textrm{\uppercase{#2}}, \textit{#1}}\par}
\newcommand{\authoronetwo}[2][]{\hspace*{9pt}{\small\textrm{\uppercase{#2}},$^{*~**}$ \textit{#1}}\par}
\newcommand{\authoronetwosame}[1]{\hspace*{9pt}{\small\textrm{\uppercase{#1}}\,$^{*~**}$ \textsc{and}}\par}
\newcommand{\authoronenoaffil}[1]{\hspace*{9pt}{\small\textrm{\uppercase{#1}}\,$^{*}$}\par}
\newcommand{\authortwonoaffil}[1]{\hspace*{9pt}{\small\textrm{\uppercase{#1}}\,$^{**}$}\par}
%%
% The address
%%
\newcommand{\addressone}[1]{\footnote{\hspace*{-14pt}$^{*}\,$Postal address: #1}\par}
\newcommand{\addresstwo}[1]{\footnote{\hspace*{-14pt}$^{**}\,$Postal address: #1}\par}
\newcommand{\addressthree}[1]{\footnote{\hspace*{-14pt}$^{***}\,$Postal address: #1}\par}
\newcommand{\addressfour}[1]{\footnote{\hspace*{-14pt}$^{****}\,$Postal address: #1}\par}
\newcommand{\addressfive}[1]{\footnote{\hspace*{-14pt}$^{*****}\,$Postal address: #1}\par}
%%
% The 'current' address (in case they've moved)
%%
\newcommand{\curaddone}[1]{\footnote{\hspace*{-14pt}$^{*}\,$Current address: #1}\par}
\newcommand{\curaddtwo}[1]{\footnote{\hspace*{-14pt}$^{**}\,$Current address: #1}\par}
\newcommand{\curaddthree}[1]{\footnote{\hspace*{-14pt}$^{***}\,$Current address: #1}\par}
\newcommand{\curaddfour}[1]{\footnote{\hspace*{-14pt}$^{****}\,$Current address: #1}\par}
\newcommand{\curaddfive}[1]{\footnote{\hspace*{-14pt}$^{*****}\,$Current address: #1}\par}
%%
%  Email address
%%
\newcommand{\email}[1]{\begin{footnotesize}Email address: #1\end{footnotesize}}
\newcommand{\emailone}[1]{\footnote{\hspace*{-14pt}$^{*}\,$Email address: #1}\par}
\newcommand{\emailtwo}[1]{\footnote{\hspace*{-14pt}$^{**}\,$Email address: #1}\par}
%%
\renewcommand{\author}{\authorone}
\newcommand{\address}{\addressone}
%%
% The abstract environment
%%
\renewenvironment{abstract}
                 {\vspace{6pt}
                  \begin{center}
                  \begin{minipage}{315.83pt}
                  \small
                  \begin{center}
                  {\bf Abstract}
                  \end{center}
                  \noindent\ignorespaces
                 }
                 {\end{minipage}\end{center}}
%%
% Keywords
%%
\newcommand{\keywords}[1]
           {\begin{center}
            \begin{minipage}{315.83pt}
            \small
            \noindent \emph{Keywords:}~{\textrm{#1}}
            \end{minipage}
            \end{center}
            \normalsize
           }
%%
% AMS classes
%%
\newcommand{\amsprimary}[1]
           {\begin{center}
            \begin{minipage}{315.83pt}
            \small
            \noindent 2000 Mathematics Subject Classification:~Primary {\uppercase{#1}}
            \end{minipage}
            \end{center}
            \par\normalsize
           }
%%
\newcommand{\ams}[2]
           {\begin{center}
            \begin{minipage}{315.83pt}
            \small
            \noindent 2000 Mathematics Subject Classification:~Primary {\uppercase{#1}}\\
            \phantom{2000 Mathematics Subject Classification:~}Secondary {\uppercase{#2}}
            \end{minipage}
            \end{center}
            \par\normalsize
           }
%%
\newcommand\msc[2]{\ams{#1}{#2}}
\newcommand\mscprimary[1]{\amsprimary{#1}}
%%
% The section headings
%%
\renewcommand{\section}{\makeatletter
\renewcommand{\@seccntformat}[1]{{\csname the##1\endcsname.}\hspace{0.45em}}
\makeatother
\@startsection
{section}%                                            the name
{1}%                                                  the level
{0pt}%                                                the indent
{\baselineskip}%                                      the beforeskip
{0.5\baselineskip}%                                   the afterskip
{\centering\normalsize\bfseries\mathversion{bold}}}%  the style
%%
\renewcommand{\subsection}{\makeatletter
\renewcommand{\@seccntformat}[1]{{\csname the##1\endcsname.}\hspace{0.45em}}
\makeatother
\@startsection
{subsection}%                                         the name
{2}%                                                  the level
{0pt}%                                                the indent
{0.5\baselineskip}%                                   the beforeskip
{0.25\baselineskip}%                                  the afterskip
{\normalsize\bfseries\mathversion{bold}}}%            the style
%%
\renewcommand{\subsubsection}{\makeatletter
\renewcommand{\@seccntformat}[1]{{\rm{\csname the##1\endcsname.}}\hspace{0.45em}}
\makeatother
\@startsection
{subsubsection}%                   the name
{3}%                               the level
{0pt}%                             the indent
{0.5\baselineskip}%                the beforeskip
{-0.25\baselineskip}%              the afterskip
{\normalsize\itshape}}%            the style
%%
%%
% Appendices
%%
\renewcommand{\appendix}{\setcounter{section}{0}\renewcommand{\thesection}{\Alph{section}}
\renewcommand{\section}{\makeatletter
\renewcommand{\@seccntformat}[1]{{\appendixname\ \csname thesection\endcsname.}\hspace{0.45em}}
\makeatother
\@startsection
{section}%                                            the name
{1}%                                                  the level
{0pt}%                                                the indent
{\baselineskip}%                                      the beforeskip
{0.5\baselineskip}%                                   the afterskip
{\centering\normalsize\bfseries\mathversion{bold}}}%  the style
}
%%
% The Acknowledgements section
%%
\newcommand\ack{\section*{Acknowledgement}}
\newcommand\Ack{\section*{Acknowledgement}}
\newcommand\acks{\section*{Acknowledgements}}
\newcommand\Acks{\section*{Acknowledgements}}
%%
% The following are commands to print a ruled space, indicating
% the position of a figure.
%%
\newcounter{figno}
\newcommand{\Fig}[1]
           {\setcounter{figno}{\value{figure}+1}
            \begin{figure}
            \begin{center}
            \begin{picture}(150,150)
            \put(0,0){\framebox(150,150){Figure \thefigno}}
            \end{picture}
            \end{center}
            \caption{\small#1}
            \end{figure}
           }
%%
\newcommand{\hFig}[1]
           {\setcounter{figno}{\value{figure}+1}
            \begin{figure}[h]
            \begin{center}
            \begin{picture}(150,150)
            \put(0,0){\framebox(150,150){Figure \thefigno}}
            \end{picture}
            \end{center}
            \caption{\small#1}
            \end{figure}
           }
%%
% The following commands refer to table captions.
%%
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{0.9}
\setlength{\textfloatsep}{10pt plus 2pt minus 2pt}
\setlength{\floatsep}{10pt plus 2pt minus 2pt}
\def\fnum@figure{\small{\sc\figurename}~\thefigure}
\def\fnum@table{\small{\sc\tablename}~\thetable}
%%
% The following commands are to do with theorem-like environments.
%%
% This bit defines the style
%%
\gdef\th@plain{\normalfont\itshape
  \def\@begintheorem##1##2{%
        \item[\hskip\labelsep \theorem@headerfont ##1\ {\bf ##2.}] }%
\def\@opargbegintheorem##1##2##3{%
   \item[\hskip\labelsep \theorem@headerfont ##1\ ##2.]{\upshape(}\emph{##3.}{\upshape)} }
}
%%
% These are the various available environments
%%
% For Theorem 1, Lemma 1, Corollary 1, Propostion 1,...
%%
\newtheorem{theorem}{\noindent Theorem}
\newtheorem{lemma}{\noindent Lemma}
\newtheorem{corollary}{\noindent Corollary}
\newtheorem{proposition}{\noindent Proposition}
\newtheorem{conjecture}{\noindent Conjecture}
\newtheorem{assertion}{\noindent Assertion}
\newtheorem{assumption}{\noindent Assumption}
\newtheorem{condition}{\noindent Condition}
%%
% For Theorem 1.1, Lemma 1.1, Corollary 1.1, Propostion 2.1,...
%%
\newtheorem{thm}{\noindent Theorem}[section]
\newtheorem{lem}{\noindent Lemma}[section]
\newtheorem{cor}{\noindent Corollary}[section]
\newtheorem{prop}{\noindent Proposition}[section]
\newtheorem{conj}{\noindent Conjecture}[section]
\newtheorem{assert}{\noindent Assertion}[section]
\newtheorem{assumpt}{\noindent Assumption}[section]
\newtheorem{cond}{\noindent Condition}[section]
%%
\theoremheaderfont{\normalfont\bfseries}
\theorembodyfont{\slshape}
\setlength{\theorempreskipamount}{6pt plus 2pt}
\setlength{\theorempostskipamount}{6pt plus 2pt}
%%
% For Example 1, Definition 1, ...
%%
{\theorembodyfont{\rmfamily} \newtheorem{example}{\noindent Example}}
{\theorembodyfont{\rmfamily} \newtheorem{definition}{\noindent Definition}}
{\theorembodyfont{\rmfamily} \newtheorem{problem}{\noindent Problem}}
{\theorembodyfont{\rmfamily} \newtheorem{observation}{\noindent Observation}}
{\theorembodyfont{\rmfamily} \newtheorem{result}{\noindent Result}}
{\theorembodyfont{\rmfamily} \newtheorem{remark}{\noindent Remark}}
{\theorembodyfont{\rmfamily} \newtheorem{remarks}[remark]{\noindent Remarks}}
{\theorembodyfont{\rmfamily} \newtheorem{note}{\noindent Note}}
{\theorembodyfont{\rmfamily} \newtheorem{notes}[note]{\noindent Notes}}
%%
% For Example 1.1, Definition 1.1, ...
%%
{\theorembodyfont{\rmfamily} \newtheorem{ex}{\noindent Example}[section]}
{\theorembodyfont{\rmfamily} \newtheorem{defn}{\noindent Definition}[section]}
{\theorembodyfont{\rmfamily} \newtheorem{prob}{\noindent Problem}[section]}
{\theorembodyfont{\rmfamily} \newtheorem{obs}{\noindent Observation}[section]}
{\theorembodyfont{\rmfamily} \newtheorem{res}{\noindent Result}[section]}
{\theorembodyfont{\rmfamily} \newtheorem{rem}{\noindent Remark}[section]}
{\theorembodyfont{\rmfamily} \newtheorem{rems}[rem]{\noindent Remarks}}
{\theorembodyfont{\rmfamily} \newtheorem{nte}{\noindent Note}[section]}
{\theorembodyfont{\rmfamily} \newtheorem{ntes}[nte]{\noindent Notes}}
%%
% For unnumbered Example, Definition, Remark,...
%%
\newenvironment{exnn}{\addvspace{\medskipamount}\noindent\textbf{Example.}}{\medbreak}
\newenvironment{defnn}{\addvspace{\medskipamount}\noindent\textbf{Definition.}}{\medbreak}
\newenvironment{probnn}{\addvspace{\medskipamount}\noindent\textbf{Problem.}}{\medbreak}
\newenvironment{obsnn}{\addvspace{\medskipamount}\noindent\textbf{Observation.}}{\medbreak}
\newenvironment{resnn}{\addvspace{\medskipamount}\noindent\textbf{Result.}}{\medbreak}
\newenvironment{remnn}{\addvspace{\medskipamount}\noindent\textbf{Remark.}}{\medbreak}
\newenvironment{remsnn}{\addvspace{\medskipamount}\noindent\textbf{Remarks.}}{\medbreak}
\newenvironment{notenn}{\addvspace{\medskipamount}\noindent\textbf{Note.}}{\medbreak}
\newenvironment{notesnn}{\addvspace{\medskipamount}\noindent\textbf{Notes.}}{\medbreak}
%%
% The proof environment
%%
\newenvironment{proof}[1][Proof]
               {\par \normalfont \topsep6\p@\@plus2\p@\relax
                \trivlist
                \item[\hspace{17pt}\itshape #1{.}]\ignorespaces
               }{\endtrivlist}
%%
% Various useful definitions
%%
\def\var{\mathop{\rm var}\nolimits}    %variance
\def\cov{\mathop{\rm cov}\nolimits}    %covariance
\def\corr{\mathop{\rm corr}\nolimits}  %correlation
%
\newcommand{\rd}{\mathrm{d}} %differential d
\DeclareMathOperator\sd{d\!} %differential d preceeded by a thin space, when needed
\newcommand{\ri}{\mathrm{i}} %imaginary i
\newcommand{\re}{\mathrm{e}} %exponential e
\DeclareMathOperator\sP{P}   %probability, treated as an operator
\newcommand{\rP}{\mathrm{P}} %probability, when spacing isn't a worry
\DeclareMathOperator\sE{E}   %expectation, treated as an operator
\newcommand{\rE}{\mathrm{E}} %expectation, when spacing isn't a worry
%
\newcommand{\trans}{^\top}   %matrix transpose
%
\newcommand{\cvgpr}{\xrightarrow{\text{\upshape\tiny P}}}   %convergence in probability
\newcommand{\cvgwk}{\xrightarrow{\text{\upshape\tiny W}}}   %weak convergence
\newcommand{\cvgdist}{\xrightarrow{\text{\upshape\tiny D}}} %convergence in distribution
\newcommand{\eqdist}{\stackrel{\text{\upshape\tiny D}}{=}}  %equality in distribution
%
\hyphenpenalty=1000
%
\chardef\ii="10
%%
% The name--date reference list style
%%
\newenvironment{harvreferences}
               {\section*{References}
                \begin{footnotesize}
                \begin{list}{}{\setlength{\itemsep}{0pt}
                               \setlength{\parsep}{0pt}
                               \setlength{\labelwidth}{0pt}
                               \setlength{\leftmargin}{12pt}
                               \setlength{\labelsep}{0pt}}
                \setlength{\itemindent}{-12pt}
               }{\end{list}\end{footnotesize}}
%%
% bold italic font for use in vectors etc
%%
\DeclareMathAlphabet{\bi}{OT1}{ptm}{b}{it}
%
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\bfeta}{\boldsymbol{\feta}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\biota}{\boldsymbol{\iota}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bupsilon}{\boldsymbol{\upsilon}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bchi}{\boldsymbol{\chi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bvarepsilon}{\boldsymbol{\varepsilon}}
\newcommand{\bvartheta}{\boldsymbol{\vartheta}}
\newcommand{\bvaromega}{\boldsymbol{\varomega}}
\newcommand{\bvarrho}{\boldsymbol{\varrho}}
\newcommand{\bvarsigma}{\boldsymbol{\varsigma}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}
\newcommand{\bpartial}{\boldsymbol{\partial}}
\newcommand{\bell}{\boldsymbol{\ell}}
\newcommand{\bimath}{\boldsymbol{\imath}}
\newcommand{\bjmath}{\boldsymbol{\jmath}}
%
\newcommand{\binfty}{\boldsymbol{\infty}}
\newcommand{\bnabla}{\boldsymbol{\nabla}}
\newcommand{\bdot}{\boldsymbol{\cdot}}
%%
% Short cuts for some commonly referenced journals
%%
\newcommand{\AAP}{\emph{Adv. Appl. Prob.}}
\newcommand{\ADM}{\emph{Ann. Discrete Math.}}
\newcommand{\AM}{\emph{Acta Math.}}
\newcommand{\AMM}{\emph{Amer. Math. Monthly}}
\newcommand{\AMS}{\emph{Ann. Math. Statist.}}
\newcommand{\AP}{\emph{Ann. Prob.}}
\newcommand{\AS}{\emph{Amer. Statistician}}
\newcommand{\ApS}{\emph{Appl. Statist.}}
\newcommand{\AnS}{\emph{Ann. Statist.}}
\newcommand{\ASM}{\emph{Acta Sci. Math.}}
%
\newcommand{\B}{\emph{Biometrika}}
\newcommand{\BAMS}{\emph{Bull. Amer. Math. Soc.}}
\newcommand{\BIMA}{\emph{Bull. Inst. Math. Appl.}}
%
\newcommand{\CB}{\emph{Comput. Bull.}}
\newcommand{\CJ}{\emph{Comput. J.}}
\newcommand{\CCERO}{\emph{Cahiers Centre Etudes Rech. Op\'erat.}}
\newcommand{\CJS}{\emph{Canad. J. Statist.}}
\newcommand{\CMA}{\emph{Comput. Math. Appl.}}
\newcommand{\CMP}{\emph{Commun. Math. Phys.}}
\newcommand{\CPAM}{\emph{Commun. Pure Appl. Math.}}
\newcommand{\CS}{\emph{Commun. Statist.}}
\newcommand{\CRA}{\emph{C. R. Acad. Sci. Paris}}
%
\newcommand{\DE}{\emph{Differential Equns}}
\newcommand{\DMJ}{\emph{Duke Math. J.}}
%
\newcommand{\E}{\emph{Econometrica}}
%
\newcommand{\IETAC}{\emph{IEEE Trans. Automatic Control}}
\newcommand{\IETC}{\emph{IEEE Trans. Commun.}}
\newcommand{\IETIT}{\emph{IEEE Trans. Inf. Theory}}
\newcommand{\IETR}{\emph{IEEE Trans. Rel.}}
\newcommand{\IJC}{\emph{Int. J. Control}}
\newcommand{\IJGT}{\emph{Int. J. Game Theory}}
\newcommand{\IJM}{\emph{Israel J. Math.}}
%
\newcommand{\JASA}{\emph{J. Amer. Statist. Soc.}}
\newcommand{\JAM}{\emph{J. Appl. Mech.}}
\newcommand{\JAMS}{\emph{J. Austral. Math. Soc.}}
\newcommand{\JAP}{\emph{J. Appl. Prob.}}
\newcommand{\JDE}{\emph{J. Differential Equns}}
\newcommand{\JET}{\emph{J. Econom. Theory}}
\newcommand{\JIMA}{\emph{J. Inst. Math. Appl.}}
\newcommand{\JISA}{\emph{J. Indian Statist. Assoc.}}
\newcommand{\JLMS}{\emph{J. London Math. Soc.}}
\newcommand{\JMA}{\emph{J. Multivar. Anal.}}
\newcommand{\JMAA}{\emph{J. Math. Anal. Appl.}}
\newcommand{\JMB}{\emph{J. Math. Biol.}}
\newcommand{\JMP}{\emph{J. Math. Phys.}}
\newcommand{\JOTA}{\emph{J. Optimization Theory Appl.}}
\newcommand{\JPE}{\emph{J. Political Econ.}}
\newcommand{\JRSS}{\emph{J. R. Statist. Soc.}}
\newcommand{\JS}{\emph{J. SIAM}}
\newcommand{\JSCS}{\emph{J. Statist. Comput. Simulation}}
\newcommand{\JSR}{\emph{J. Statist. Res.}}
\newcommand{\JTB}{\emph{J. Theoret. Biol.}}
\newcommand{\JTSA}{\emph{J. Time Series Anal.}}
%
\newcommand{\MAMS}{\emph{Mem. Amer. Math. Soc.}}
\newcommand{\MB}{\emph{Math. Biosci.}}
\newcommand{\MC}{\emph{Math. Comput.}}
\newcommand{\MF}{\emph{Math. Finance}}
\newcommand{\MN}{\emph{Math. Nachr.}}
\newcommand{\MOR}{\emph{Math. Operat. Res.}}
\newcommand{\MS}{\emph{Management Sci.}}
%
\newcommand{\NMJ}{\emph{Nagoya Math. J.}}
\newcommand{\N}{\emph{Nature}}
\newcommand{\NRLQ}{\emph{Naval Res. Logist. Quart.}}
%
\newcommand{\OR}{\emph{Operat. Res.}}
\newcommand{\ORQ}{\emph{Operat. Res. Quart.}}
%
\newcommand{\PTRF}{\emph{Prob. Theory Rel. Fields}}
\newcommand{\PTRS}{\emph{Phil. Trans. R. Soc.}}
\newcommand{\PAMS}{\emph{Proc. Amer. Math. Soc.}}
\newcommand{\PCPS}{\emph{Proc. Camb. Phil. Soc.}}
\newcommand{\PLMS}{\emph{Proc. London Math. Soc.}}
\newcommand{\PNAS}{\emph{Proc. Nat. Acad. Sci. USA}}
\newcommand{\PRS}{\emph{Proc. R. Soc.}}
%
\newcommand{\QAM}{\emph{Quart. Appl. Math.}}
\newcommand{\QS}{\emph{Queueing Systems}}
%
\newcommand{\RES}{\emph{Rev. Econ. Stud.}}
\newcommand{\RISI}{\emph{Rev. Int. Statist. Inst.}}
\newcommand{\RSA}{\emph{Rev. Statist. Appl.}}
%
\newcommand{\Sa}{\emph{Sankhy\=a}}
\newcommand{\SJAM}{\emph{SIAM J. Appl. Math.}}
\newcommand{\SJMA}{\emph{SIAM J. Math. Anal.}}
\newcommand{\SN}{\emph{Statist. Neerlandica}}
\newcommand{\SPA}{\emph{Stoch. Proc. Appl.}}
\newcommand{\SR}{\emph{SIAM Rev.}}
%
\newcommand{\TAMS}{\emph{Trans. Amer. Math. Soc.}}
\newcommand{\TPA}{\emph{Theory Prob. Appl.}}
\newcommand{\TPB}{\emph{Theoret. Popn Biol.}}
%
\newcommand{\ZW}{\emph{Z. Wahrscheinlichkeitsth.}}
%%
%%

